Optimization is Not Enough: Why Problem Formulation Deserves Equal Attention

Black-box optimization is increasingly used in engineering design problems where simulation-based evaluations are costly and gradients are unavailable. In this context, the optimization community has largely analyzed algorithm performance in context-free setups, while not enough attention has been devoted to how problem formulation and domain knowledge may affect the optimization outcomes. We address this gap through a case study in the topology optimization of laminated composite structures, formulated as a black-box optimization problem. Specifically, we consider the design of a cantilever beam under a volume constraint, intending to minimize compliance while optimizing both the structural topology and fiber orientations. To assess the impact of problem formulation, we explicitly separate topology and material design variables and compare two strategies: a concurrent approach that optimizes all variables simultaneously without leveraging physical insight, and a sequential approach that optimizes variables of the same nature in stages. Our results show that context-agnostic strategies consistently lead to suboptimal or non-physical designs. In contrast, the sequential strategy yields better-performing and more interpretable solutions. These findings underscore the value of incorporating, when available, domain knowledge into the optimization process and motivate the development of new black-box benchmarks that reward physically informed and context-aware optimization strategies.

==> lamination_parameters.tex <==
\section{Lamination Parameters}
\label{sec:Appx_Lamination_Parameters}
\subsection{Main Definition}

For symmetric composite laminates, the in-plane stiffness behavior can be fully characterized by four lamination parameters \( V_1, V_2, V_3, V_4 \), defined as:
\\
%
\begin{align*}
V_1 = \frac{1}{2} \int_{-1/2}^{1/2} \cos(2\theta(\hat{z})) \,  d\hat{z} & \, ,  &
V_2 = \frac{1}{2} \int_{-1/2}^{1/2} \sin(2\theta(\hat{z})) \,  d\hat{z} \\
V_3 = \frac{1}{2} \int_{-1/2}^{1/2} \cos(4\theta(\hat{z})) \,  d\hat{z} & \, ,  &
V_4 = \frac{1}{2} \int_{-1/2}^{1/2} \sin(4\theta(\hat{z})) \,  d\hat{z}, \\
\end{align*}
%
where \( \theta(\hat{z}) \) denotes the fiber orientation angle at the normalized thickness coordinate \( \hat{z} = z/h \), with \( h \) the total laminate thickness.

In the special case of \emph{balanced laminates}, each ply oriented at angle \( \theta \) is paired with another at angle \( -\theta \), symmetrically located concerning the midplane. This implies that the fiber orientation distribution satisfies the relation \( \theta(-\hat{z}) = -\theta(\hat{z}) \), i.e., it is an odd function of \( \hat{z} \).

Using the identities
\[
\sin(2\theta(-\hat{z})) = -\sin(2\theta(\hat{z})), \quad \sin(4\theta(-\hat{z})) = -\sin(4\theta(\hat{z})),
\]
since both \( \sin(2\theta(\hat{z})) \) and \( \sin(4\theta(\hat{z})) \) are odd functions over the interval \( [-1/2, 1/2] \), their integrals vanish:
\[
V_2 = \frac{1}{2} \int_{-1/2}^{1/2} \sin(2\theta(\hat{z})) \, d\hat{z} = 0, \quad
V_4 = \frac{1}{2} \int_{-1/2}^{1/2} \sin(4\theta(\hat{z})) \, d\hat{z} = 0.
\]

As a result, for balanced symmetric laminates, only \( V_1 \) and \( V_3 \) may take nonzero values, and the lamination parameter vector simplifies to:
\[
V = (V_1,V_3).
\]

This reduction not only decreases the dimensionality of the design space but also enforces laminate balance, which eliminates coupling effects such as extension–twist and bending–twist. Optimisation in this reduced parameter space remains convex and thus well-suited for efficient numerical solution techniques.

\subsection{Miki Lamination Diagram and Lamination Parameter Interpolation}

The Miki Lamination Diagram \cite{miki_optimum_1993} defines the set of all physically attainable lamination parameters \( (V_1, V_3) \) for symmetric and balanced laminates. 

\begin{figure}[htbp]
    \centering
    \input{Tikzplots/miki_diagram_repr1}
    \caption{Miki's Lamination Diagram. Adapted from \cite{serhat_lamination_2019}.}
    \label{fig:Miki_Lamination_Diagram_1}
\end{figure}

The feasible region of \( (V_1, V_3) \) values—commonly visualized through the Miki diagram—is a bounded, convex domain shown in Figure \ref{fig:Miki_Lamination_Diagram_1} as the light-gray shaded region. Each point within this region corresponds to a valid stacking sequence, with boundary points typically representing laminates made from only two fiber orientations (e.g., \( \pm\theta_1 \) and \( \pm\theta_2 \)). The interior points represent laminates with a broader distribution of fiber angles.

To interpolate within this feasible region and construct continuous laminate representations from discrete stacking configurations, the concept of \textit{volumetric ratio} is introduced. For a laminate composed of $n$ different fiber orientations \( \{ \theta_i \}_{i=1}^n \), the volumetric ratio \( \rho_i \in [0,1] \) denotes the fraction of the total thickness occupied by plies at orientation \( \theta_i \), such that:

\[
\sum_{i=1}^n \rho_i = 1.
\]

Using this ratio, the lamination parameters can be expressed as a convex combination:

\[
\begin{pmatrix}
V_1 \\
V_3
\end{pmatrix}
= \sum_{i=1}^n \rho_i
\begin{pmatrix}
\cos(2\theta_i) \\
\cos(4\theta_i)
\end{pmatrix}.
\]

This interpolation framework allows smooth mapping between stacking sequences and their corresponding lamination parameters, and vice versa. It facilitates gradient-based optimization by maintaining continuity, while ensuring that all generated designs remain inside the feasible region defined by the Miki diagram.


%% This is a plot similar to Gokhan's plot to define relationship 
\begin{figure}[htbp]
    \centering
    \input{Tikzplots/miki_diagram_interp1}
    \caption{Exemplary design with ($R_l= 0.75$, $R_r=0.25$), $P_1 (V_1,V_3) =  (-0.1768,-0.75 )$ and $P_2(V_1,V_3)=(-0.4677, 0.75)$. Adapted from \cite{serhat_lamination_2019}.}
    \label{fig:Miki_Lamination_Diagram_Interpolation_1}
\end{figure}

In design applications, optimization is often constrained to lie on the boundary of the Miki diagram, such as along the linear path \( V_3 = 2V_1 - 1 \), which has been observed to yield near-optimal solutions for many structural objectives. Once an optimal point is found in lamination parameter space, volumetric ratios can be used to reconstruct an approximate stacking sequence that realizes the desired stiffness behavior.






